String theory applications in gravitational problems and gauge theories

In this dissertation, we review the study of quark and monopole bound-state potentials within the gauge/gravity correspondence. Their behaviors often differ from what is expected on general physical grounds and field-theory considerations. We identify the configurations of physical interest by examining the stability of the string (brane) solutions dual to the flux tubes between the bound states. In particular, we formulate and prove several general statements concerning the perturbative stability of such string (brane) solutions, relevant for these configurations in a general class of backgrounds. We apply the results to N = 4 SYM and N = 1 at finite temperature and at generic points of the Coulomb branch. In all cases, the problematic regions are found to be unstable and hence physically irrelevant.

==> WilsonLoops.tex <==
\rm{Σε αυτό το κεφάλαιο θα εισάγουμε την έννοια του βρόχου \en
Wilson (Wilson-loop) \gr ο οποίος θα μας χρειαστεί αργότερα για τον
υπολογισμό ενεργειών δέσμιων καταστάσεων.}

\no
Τα κουάρκ στην \en QCD \gr χωρίζονται σε:

$\bullet$ Θεμελιώδη: ελαφρά κουάρκ,  τα οποία εμφανίζονται στην δράση

$\bullet$ Εξωτερικές προσθήκες: (απείρως) βαριά κουάρκ που
τα αποκαλώ εξωτερικά (δεν \phantom{xxxxxxx} υπάρχουν στην δράση)

\no
Στη \en QCD, \gr τα ελαφριά κουάρκ δεν βρίσκονται
ποτέ ελεύθερα στο κενό, αλλά πάντα σε δέσμιες καταστάσεις.
Για παράδειγμα, σχηματίζοντας ζεύγη με αντικουάρκ.
\no
Αφού τα εξωτερικά κουάρκ είναι πολύ βαριά, η απόσταση μεταξύ του ζεύγους
$q\bar{q}$ δεν παραμείνει σταθερή με το χρόνο. Θέλουμε να υπολογίσουμε
το δυναμικό αλληλεπίδρασης μεταξύ των δύο κουάρκ, $V_{q\bar{q}}(L)$ και για αυτό
χρειαζόμαστε κάποιο φυσικό μέγεθος που δεν θα εξαρτάται απο την βαθμίδα.
Μια σημαντική ποσότητα η οποία δεν εξαρτάται απο την βαθμίδα στις θεωρίες
\en Yang-Mills \gr είναι ο βρόχος \en Wilson \cite{Peskin} \gr
\ba
\label{2-1}
W(C;R)=Tr_R[P e^{i\oint_C A}],
\ea
ο οποίος δίνεται απο ένα εκθετικό διατασσόμενης διαδρομής (\en path ordered) \gr
πάνω στο πεδίο βαθμίδας, κατά μήκος μιας κλειστής τροχιάς $C$ ενώ το ίχνος έχει παρθεί
πάνω σε μια τυχαία αναπαράσταση $R$ του πεδίου βαθμίδας. Θα αποδείξουμε ότι η
ποσότητα αυτή δεν εξαρτάται από μετασχηματισμούς βαθμίδας.
\no
Θεωρούμε ένα μη αβελιανό πεδίο $A_\mu\equiv A_\mu^\a T_\a$, όπου $T_\a$
είναι οι γεννήτορες της μη αβελιανής ομάδας $G$ στην οποία παίρνει τιμές το $A_\mu$.
Οι μετασχηματισμοί βαθμίδας αυτού του μη αβελιανού πεδίου είναι
\ba
\label{2-2}
A_\mu\to\Om(x)A_\mu\Om^{-1}(x)-i(\del_\mu\Om)\Om^{-1}\ .
\ea
Ο απειροστός μετασχηματισμός $\Om(x)=e^{i\chi(x)}$ για μικρά $\chi(x)=\chi^aT_a$
ισούται με
\ba
\label{2-3}
\d A_\mu=\del_\mu\chi-i[A_\mu,\chi]
\ea
και το οποίο συνεπάγεται
\ba
\label{2-4}
&&e^{iA_\mu d\xi^\mu}\simeq(1+iA_\mu d\xi^\mu)\to
1+i\Om(x)A_\mu d\xi^\mu\Om^{-1}(x)+d\xi^\mu(\del_\mu\Om)\Om^{-1}\nonumber \\
&&=[\Om(x)(1+iA_\mu d\xi^\mu)+d\xi^\mu\del_\mu\Om(x)]\Om^{-1}(x)\nonumber \\
&&\simeq\Om(x+dx)(1+iA_\mu d\xi^\mu)\Om^{-1}(x)\simeq\Om(x+dx)e^{iA_\mu d\xi^\mu}\Om^{-1}(x)\ .
\ea
\no
Με την βοήθεια της Εξ. \eqn{2-4} έχουμε ότι
\ba
\label{2-5}
P e^{\oint_C A}\to\Om(x)P e^{\oint_C A}\Om^{-1}(x)\ .
\ea
\no
Παρατηρούμε όμως ότι το ίχνος της Εξ. \eqn{2-5} παραμένει αναλλοίωτο,
επομένως και ο βρόχος \en Wilson $W(C;R)$ \gr Εξ. \eqn{2-1}.\\
\no
Από την αναμενόμενη τιμή του βρόχου \en Wilson $W(C;R)$ \gr μπορούμε να υπολογίσουμε
το δυναμικό αλληλεπίδρασης. Για το σκοπό αυτό θεωρούμε ένα ορθογώνιο παραλληλόγραμμο
στο ευκλείδιο χώρο $t-x$, με μήκος $T$ κατά μήκος του χρόνου $t$ και μήκος $L$
κατά μήκος του χώρου $x$. Η Εξ. \eqn{2-1} ισούται με ένα άθροισμα
σε όλες τις ενέργειες και για μεγάλα $T$ ($Τ\gg L$) η αναμενόμενη τιμή
συμπεριφέρεται ως $e^{-TE}$, όπου $E$ είναι η ελάχιστη ενέργεια του ζεύγους
κουάρκ και αντικουάρκ. Οπότε, βρίσκουμε ότι μια εναλλακτική
σχέση για την αναμενόμενη τιμή του βρόχου \en Wilson \gr
\ba
\label{2-6}
<W(c)>\ \simeq e^{-TV(L)}\ ,
\ea
\no
όπου $V(L)$ είναι το δυναμικό κουάρκ και αντικουάρκ.
Όπως θα δούμε αργότερα για μεγάλα $N$ και μεγάλες τιμές του $g_{YM}^2N$,
μέσω της αναλογίας \en AdS/CFT \gr ο υπολογισμός του $<W>$ της \en CFT
\gr γίνεται από την ελαχιστοποίηση μιας επιφάνειας στον χώρο $AdS$.

